Step by Step Loss Goes Very Far: Multi-Step Quantization for Adversarial Text Attacks

We propose a novel gradient-based attack against transformer-based language models that searches for an adversarial example in a continuous space of token probabilities. Our algorithm mitigates the gap between adversarial loss for continuous and discrete text representations by performing multi-step quantization in a quantization-compensation loop. Experiments show that our method significantly outperforms other approaches on various natural language processing (NLP) tasks.

==> content/tables/extended_main_results.tex <==
% \begin{table*}[t!]
% \centering
% \small
% \begin{tabular}{|l|cc|cc|cc|cc|cc|}
% \hline
%  & \multicolumn{2}{|c|}{\textbf{AG News}} & \multicolumn{2}{|c|}{\textbf{Yelp}} & \multicolumn{2}{|c|}{\textbf{IMDB}} & 
%  \multicolumn{2}{|c|}{\textbf{MNLI p.}} & \multicolumn{2}{|c|}{\textbf{MNLI h.}} \\
% \textbf{Attack} & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.}  & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.}\\

% \hline
% Naive & 102 & 0.873 & 102 & 0.842 & 100 & 0.829 & 97 & 0.943 & 97 & 0.934 \\
% GBDA & 1098 & 0.798 & 1101 & 0.814 & 1082 & 0.794 & 1044 & 0.869 & 1044 & 0.891 \\
% MANGO & 496 & 0.831 & 1128 & 0.801 & 1647 & 0.834 & 326 & 0.914 & 258 & 0.926 \\

% \hline
% TextFooler & 330 & 0.825 & 479 & 0.925 & 725 & 0.931 & - & - & 74 & 0.953 \\
% Bert-Attack & 620 & 0.863 & 665 & 0.943 & 900 & 0.958 & 146 & 0.957 & 95 & 0.968 \\
% BAE & 259 & 0.884 & 427 & 0.939 & 585 & 0.954 & 92 & 0.957 & 69 & 0.971 \\
% black MANGO & 3728 & 0.667 & 2803 & 0.692 & 3142 & 0.661 & 3158 & 0.84 & 3387 & 0.891 \\

% \hline
% \end{tabular}
% \caption{\label{tab:extended_main_results}
% Comparison of the white-box (top) and black-box (bottom) attacks. We report the average number of queries to the attacked model ("\#") and the average BERTScore between the attacked and perturbed texts ("BERT S."). In MNLI p., an attack is allowed to modify only the premise, while in MNLI h., only the hypothesis. We omit results for TextFooler on MNLI p., as it has not generated any adversarial example.
% }
% \end{table*}

\begin{table*}[t!]
\centering
\small
\begin{tabular}{|l|cc|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{|c|}{\textbf{AG News}} & \multicolumn{2}{|c|}{\textbf{Yelp}} & \multicolumn{2}{|c|}{\textbf{IMDB}} & 
 \multicolumn{2}{|c|}{\textbf{MNLI p.}} & \multicolumn{2}{|c|}{\textbf{MNLI h.}} \\
\textbf{Attack} & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.}  & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.} & \textbf{\#} & \textbf{BERT S.}\\

\hline
TextFooler & 330 & 0.825 & 479 & 0.925 & 725 & 0.931 & - & - & 74 & 0.953 \\
Bert-Attack & 620 & 0.863 & 665 & 0.943 & 900 & 0.958 & 146 & 0.957 & 95 & 0.968 \\
BAE & 259 & 0.884 & 427 & 0.939 & 585 & 0.954 & 92 & 0.957 & 69 & 0.971 \\
black MANGO & 3728 & 0.667 & 2803 & 0.692 & 3142 & 0.661 & 3158 & 0.84 & 3387 & 0.891 \\

\hline
Naive & 102 & 0.873 & 102 & 0.842 & 100 & 0.829 & 97 & 0.943 & 97 & 0.934 \\
GBDA & 1098 & 0.798 & 1101 & 0.814 & 1082 & 0.794 & 1044 & 0.869 & 1044 & 0.891 \\
MANGO & 496 & 0.831 & 1128 & 0.801 & 1647 & 0.834 & 326 & 0.914 & 258 & 0.926 \\

\hline
\end{tabular}
\caption{\label{tab:extended_main_results}
Comparison of the black-box (top) and white-box (bottom) attacks. We report the average number of queries to the attacked model ("\#") and the average BERTScore between the attacked and perturbed texts ("BERT S."). In MNLI p., an attack is allowed to modify only the premise, while in MNLI h., only the hypothesis. We omit results for TextFooler on MNLI p., as it has not generated any adversarial example.
}
\end{table*}

==> content/tables/main_results.tex <==
% \begin{table*}[t!]
% \centering
% \small
% \begin{tabular}{l|cc|cc|cc|cc|cc}
% \hline
%  & \multicolumn{2}{|c|}{\textbf{AG News}} & \multicolumn{2}{|c|}{\textbf{Yelp}} & \multicolumn{2}{|c|}{\textbf{IMDB}} & 
%  \multicolumn{2}{|c|}{\textbf{MNLI p.}} & \multicolumn{2}{|c}{\textbf{MNLI h.}} \\

% \textbf{Attack} & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.}  & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.}\\

% \hline
% Naive & 43.7 & 0.823 & 35.1 & 0.819 & 30.5 & 0.855 & 31.6 & 0.925 & 8.4 & 0.910 \\
% GBDA & 12.9 & 0.722 & \textbf{4.5} & 0.787 & 6.3 & 0.826 & 5.9 & 0.837 & 0.6 & 0.843 \\
% MANGO & \textbf{2.7} & 0.783 & 8.5 & 0.815 & \textbf{0.3} & 0.878 & \textbf{2.4} & 0.897 & \textbf{0.3} & 0.905 \\

% \hline
% TextFooler & 20.8 & 0.811 & 5.7 & 0.924 & 1.1 & 0.947 & - & - & 8.6 & 0.943 \\
% Bert-Attack & 20.1 & 0.829 & \textbf{1.9} & 0.934 & \textbf{0.6} & 0.957 & \textbf{3.9} & 0.930 & \textbf{2.6} & 0.952 \\
% BAE & 50.1 & 0.875 & 11.9 & 0.937 & 8.7 & 0.965 & 16.0 & 0.930 & 7.0 & 0.954 \\
% black MANGO & \textbf{9.7} & 0.574 & 15.7 & 0.618 & 8.6 & 0.653 & 35.1 & 0.808 & 9.1 & 0.854 \\

% \hline
% \textbf{Original Accuracy} & 
% \multicolumn{2}{|c|}{99.6} &  
% \multicolumn{2}{|c|}{99.9} & 
% \multicolumn{2}{|c|}{98.2} & 
% \multicolumn{2}{|c|}{94.7} & 
% \multicolumn{2}{|c}{94.7} \\
% \hline
% \end{tabular}
% \caption{\label{tab:main_results}
% Training accuracy of BERT model under attack ("Adv.") and the average similarity of perturbed texts ("Sim.") computed with USE \cite{use} for white-box (top) and black-box (bottom) attacks. The best result in every column is \textbf{bold}. We omit results for TextFooler on MNLI p., as it has not generated any adversarial example. Our MANGO method achieves superior results on most tasks, while maintaining high semantic similarity.
% }
% \end{table*}

\begin{table*}[t!]
\centering
\small
\begin{tabular}{l|cc|cc|cc|cc|cc}
\hline
 & \multicolumn{2}{|c|}{\textbf{AG News}} & \multicolumn{2}{|c|}{\textbf{Yelp}} & \multicolumn{2}{|c|}{\textbf{IMDB}} & 
 \multicolumn{2}{|c|}{\textbf{MNLI p.}} & \multicolumn{2}{|c}{\textbf{MNLI h.}} \\

\textbf{Attack} & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.}  & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.} & \textbf{Adv.} & \textbf{Sim.}\\

\hline
TextFooler & 20.8 & 0.811 & 5.7 & 0.924 & 1.1 & 0.947 & - & - & 8.6 & 0.943 \\
Bert-Attack & 20.1 & 0.829 & \textbf{1.9} & 0.934 & 0.6 & 0.957 & 3.9 & 0.930 & 2.6 & 0.952 \\
BAE & 50.1 & 0.875 & 11.9 & 0.937 & 8.7 & 0.965 & 16.0 & 0.930 & 7.0 & 0.954 \\
black MANGO & 9.7 & 0.574 & 15.7 & 0.618 & 8.6 & 0.653 & 35.1 & 0.808 & 9.1 & 0.854 \\

\hline
Naive & 43.7 & 0.823 & 35.1 & 0.819 & 30.5 & 0.855 & 31.6 & 0.925 & 8.4 & 0.910 \\
GBDA & 12.9 & 0.722 & 4.5 & 0.787 & 6.3 & 0.826 & 5.9 & 0.837 & 0.6 & 0.843 \\
MANGO & \textbf{2.7} & 0.783 & 8.5 & 0.815 & \textbf{0.3} & 0.878 & \textbf{2.4} & 0.897 & \textbf{0.3} & 0.905 \\

\hline
\textbf{Original Accuracy} & 
\multicolumn{2}{|c|}{99.6} &  
\multicolumn{2}{|c|}{99.9} & 
\multicolumn{2}{|c|}{98.2} & 
\multicolumn{2}{|c|}{94.7} & 
\multicolumn{2}{|c}{94.7} \\
\hline
\end{tabular}
\caption{\label{tab:main_results}
Training accuracy of BERT model under attack ("Adv.") and the average similarity of perturbed texts ("Sim.") computed with USE \cite{use} for black-box (top) and white-box (bottom) attacks. The best results are \textbf{bold}. We omit results for TextFooler on MNLI p., as it has not generated any adversarial example. Our MANGO method achieves superior results on most tasks, while maintaining high semantic similarity.
}
\end{table*}
